GMap: Drawing Graphs as Maps

Information visualization is essential in making sense out of large data sets. Often, high-dimensional data are visualized as a collection of points in 2-dimensional space through dimensionality reduction techniques. However, these traditional methods often do not capture well the underlying structural information, clustering, and neighborhoods. In this paper, we describe GMap: a practical tool for visualizing relational data with geographic-like maps. We illustrate the effectiveness of this approach with examples from several domains All the maps referenced in this paper can be found in http://www.research.att.com/~yifanhu/GMap

==> abstract.tex <==
Information visualization is essential in making sense out of large
data sets. Often, high-dimensional data are visualized as a collection
of points in 2-dimensional space through dimensionality reduction
techniques.  However, these traditional methods often do not capture well 
the underlying structural information, clustering, and neighborhoods. In this paper, we
describe \gmap: a practical tool for visualizing relational data with 
geographic-like maps. We illustrate the
effectiveness of this approach with examples from several domains
All the maps referenced in this paper can be found in \url{www.research.att.com/~yifanhu/GMap}.


==> intro.tex <==
\section{Introduction}

Graphs capture relationships between objects and graph drawing allows us to visualize such relationships. Typically vertices are
placed as points in two or three dimensional space, and edges are represented as lines between the corresponding vertices. The layout optimizes some aesthetic criteria,
for example, minimal edge length and edge crossings. While such point-and-line representation are most commonly used, other representations have also been
considered. For example, treemaps~\cite{treemaps92}
use a recursive space filling approach to represent trees. There is also a large body of work on representing planar graphs as {\em
contact graphs}~\cite{He99,Liao03,FMR04}, where vertices are embodied by geometrical objects and edges are shown by two objects touching in some specified fashion. 
Koebe's theorem~\cite{Koebe36} shows that
all planar graphs can be represented by touching disks.
Similar representation is possible with triangles, where two adjacent vertices correspond to vertex-to-side touching pair of triangles, as shown by de Fraysseix {\em et al.}~\cite{FMR04}. 
If vertices are represented by rectilinear regions and edges correspond to side-to-side contact between paired regions, He~\cite{He99} has shown that all planar graphs have such drawings.
%Recently, it was shown that all planar graphs can be represented by %touching convex hexagons, where an
%edge corresponds to two pairs of hexagons with non-trivially %overlapping sides~\cite{Gansner_Hu_Kobourov_2009}.  
%Rectanguar node shape is possible
%for some planar graphs~\cite{Buchsbaum08}.  
Graph representations of side-to-side touching regions tend to be visually appealing and have the added advantage that they suggest the familiar metaphor of a geographical map.
%{\bf Here we should include some examples of planar graphs drawn 
%with the ESA algorithm.}
 
In this paper we describe \gmap, an algorithm to represent general graphs as 
maps.
%, in other words, touching polygons of arbitrary shape/size. 
Clearly, there are theoretical limitations to what graphs can be 
represented exactly by touching polygons, even when allowing for non-convexity. 
However, our aim here is practical rather than graph theoretical. 
We do not insist that the created map be an exact representation of the graph 
but that it captures the underlying relationships well. With this in mind, 
we do not insist that all vertices are represented by individual polygons either. 
In fact, we group closely connected vertices into regions. If we would like to show 
all of the relationships, we can superimpose a graph drawing on top of the map. 
%{\bf Here we should include a map which illustrates that well.}

Our overall goal is to create a representation which makes the
underlying data understandable and visually appealing. Our map
representation is especially effective when the underlying graph
contains structural information such as clusters and/or hierarchy. The
traditional line-and-point representation of graphs often requires
considerable effort to comprehend, and often puts off general users.
On the other hand, a map representation is more intuitive, as most
people are very familiar with maps and even enjoy carefully examining
maps.

%Our map representation is especially effective when the underlying %graph contains structural information such as clusters and/or %hierarchy.
%that are difficult to visualize. 
%We propose to use maps to explicitly
%defining the boundary of the clusters and coloring the regions, thus %making
%the clustering information clear. 

Given that we do not insist on the map to be an exact representation
for the graph, at first it may seem trivial to generate a map. For
example, one can start with a ``good'' graph drawing and build a
Voronoi diagram of the vertices along with the four corners of the
bounding box for the drawing. However, the results are visually
unappealing as maps, with straight borders between ``countries'' and
jagged, angular overall appearance. 
%{\bf Do we have some old images of such maps?}
%and outer boundaries with sharper corners.  
Our \gmap\ algorithm takes as input a graph and produces a 
map with a ``natural'' look, outer boundaries that follow the outline of the vertex sets, and
inner boundaries having the twists and turns found in real
maps. Our maps also can have lakes, islands, and peninsulas, similar to those found in real geographic maps; see Figures~\ref{gd_map}-\ref{map_1984}.\footnote{
This paper contains zoom-able high resolution images; all the images are also available at \url{www.research.att.com/~yifanhu/GMap}.}

% {\bf Perfect place for an image of a ``good'' map we've generated.} %We call such a map representation of a graph GMap.




==> related.tex <==
\section{Related Work}


There is little previous work on generating map representations of graphs. Most related work deals with accurately and appealingly representing a given geographic region, or on re-drawing an 
existing map subject to additional constraints. Examples of 
the first kind of problem are found in traditional cartography, e.g., the 1569 Mercator projection of the sphere into 2D Euclidean space.
Examples of the second kind of problem are found in cartograms, where the goal is to redraw a map so that the 
country areas are proportional to some metric, an idea which dates back to 1934~\cite{Raisz34} and is
still popular today (e.g., the New York Times red-blue maps of the US, showing the presidential election results in 2000 and 2004 with states drawn proportional to population). 

The map of science~\cite{mapofscience} uses vertex coloring in a graph drawing to provide an overview of the scientific landscape, based on citations of journal articles.
Treemaps~\cite{treemaps92}, squarified treemaps~\cite{squarified} and the more recent newsmaps~\cite{newsmap} represent hierarchical information by means of space-filling tilings, allocating area proportional to some important metric. 
%The map of New Yorkistan~\cite{newyorkistan} takes a real place, New %York City, and creatively renames its neighborhoods. 
%Concept maps are diagrams showing relationships among %concepts~\cite{conceptmap}. Somewhat similar are cognitive maps and mind-maps %used to represent words or ideas linked to and arranged around a central key %word~\cite{mindmap}. Popular among recent such subway-like maps are the web %trend maps~\cite{webtrendmap}.  

%The map of New Yorkistan~\cite{newyorkistan} takes a real place, New %York %City, and creatively renames its neighborhoods. 

Representing imagined places on a map as if they were real countries also has a long history,  e.g., the 1930's Map of Middle Earth by Tolkien~\cite{tolkien} and the B{\"u}cherlandes map by Woelfle from the same period~\cite{woelfle}.
More recent popular maps include xkcd's
Map of Online Communities~\cite{xkcd}. While most such maps are 
generated in an ad hoc manner and are not 
strictly based on underlying data, they are often visually 
appealing.

Generating synthetic geography has a large literature, connected to its use in computer games and movies. Most of the work (e.g.,\cite{Musgrave_93, %Pabst_jense, 
Liao_petrou_zhao}) relies on
variations of a fractal model. Although these techniques could provide additional photorealism,
it is unclear how they could be used with the position and size constraints attached to the maps
we consider here.

